Generating event descriptions under syntactic and semantic constraints

With the goal of supporting scalable lexical semantic annotation, analysis, and theorizing, we conduct a comprehensive evaluation of different methods for generating event descriptions under both syntactic constraints -- e.g. desired clause structure -- and semantic constraints -- e.g. desired verb sense. We compare three different methods -- (i) manual generation by experts; (ii) sampling from a corpus annotated for syntactic and semantic information; and (iii) sampling from a language model (LM) conditioned on syntactic and semantic information -- along three dimensions of the generated event descriptions: (a) naturalness, (b) typicality, and (c) distinctiveness. We find that all methods reliably produce natural, typical, and distinctive event descriptions, but that manual generation continues to produce event descriptions that are more natural, typical, and distinctive than the automated generation methods. We conclude that the automated methods we consider produce event descriptions of sufficient quality for use in downstream annotation and analysis insofar as the methods used for this annotation and analysis are robust to a small amount of degradation in the resulting event descriptions.

==> figures/experiment-1-naturalness/surveyflow.tex <==
% surveyflow.tex
\usetikzlibrary{shapes, arrows.meta, positioning}

\tikzstyle{startstop} = [rectangle, rounded corners, minimum width=2cm, minimum height=1cm, text centered, draw=black, fill=red!30]
\tikzstyle{io} = [rectangle, minimum width=2cm, minimum height=1cm, text centered, draw=black, fill=blue!30]
\tikzstyle{process} = [rectangle, minimum width=2cm, minimum height=1cm, text centered, draw=black, fill=orange!30]
\tikzstyle{decision} = [diamond, minimum width=2cm, minimum height=1cm, text centered, draw=black, fill=green!30]
\tikzstyle{arrow} = [thick,->,>=stealth]

\begin{tikzpicture}[node distance=1.5cm, every node/.style={text width=3cm, align=center}]

% Layer 1
\node (start) [startstop] {Start};
\node (intro) [io, right=of start] {Introduction};
\node (introQ) [process, right=of intro] {Guided Questions};

% Layer 2
\node (calibrationQ) [process, below=of start] {Calibration Questions};
\node (mainQ) [process, right=of calibrationQ] {Main Questions};
\node (end) [startstop, right=of mainQ] {End};

% Arrows
\draw [arrow] (start) -- (intro);
\draw [arrow] (intro) -- (introQ);
\draw [arrow] (introQ) -- (calibrationQ);
\draw [arrow] (calibrationQ) -- (mainQ);
\draw [arrow] (mainQ) -- (end);

\end{tikzpicture}


==> sections/experiments-naturalness-and-typicality.tex <==
Having gathered three sets of sentences (from Reddit; from the LLM prompted with its own sense glosses; from the LLM prompted with the PropBank sense glosses), we elicited human ratings of their naturalness and typicality. 
We ran six experiments in total, one for naturalness and one for typicality for each of the three sets of sentences.   We present both tasks before turning to their results.


\subsection{Naturalness}

In the studies of naturalness, participants are asked to rate the naturalness of each sentence on a continuous scale ranging from \textit{extremely unnatural} to \textit{perfectly natural} (Figure \ref{fig:instr_exp}).  They are instructed that ``a natural sentence is something that a native speaker of English would naturally and fluently say, following the implicit structural rules of English.'' They are told that \ref{sleep1} is natural, \ref{sleep2} is ``somewhat natural, because -- even though it doesn't make sense (toothbrushes don't sleep) -- it does follow the structural rules of English;'' and \ref{sleep3} is unnatural. 

\ex. \label{sleep} \a. \label{sleep1} The baby seems to be sleeping.
    \b. \label{sleep2} The toothbrush seems to be sleeping. 
    \c.  \label{sleep3} The baby seems sleep to be.



Next, participants rate three practice questions similar to \ref{sleep} which they have to get right (rating the sentences like \ref{sleep1}--\ref{sleep2} above the midpoint, and the one like \ref{sleep3} below the midpoint) in order to continue.  Then they rate eight calibration sentences, those found in our norming study to be closest to the Gaussian center, from among the normed ``handwritten control'' sentences \ref{handwritten}.  Finally, they rate 89 more sentences,  
 of which a slight majority ($<59$) are target items (the rest are calibration items, used to pad the surveys to a constant length, and to encourage participants to use the full range of the scale). To generate these 89 sentences, we split all target items into about a dozen lists, with about 50 target items each. Then, the ordered calibration items are added to bring the total up to 89 items. In total, each generation procedure generates  twelve such lists, from which participants are randomly assigned to one.



\subsection{Typicality}

In the studies of typicality, participants rate the typicality of the situation described by a sentence on a continuous scale ranging from \textit{very atypical} to \textit{very typical}.   They are instructed that ``a typical situation is one in which individuals and their actions follow our normal expectations.''  They are told that \ref{cooked1} describes a typical situation, while \ref{cooked2} is less typical because ``waitresses typically serve food instead of cooking it and salads are not cooked;'' and \ref{cooked3} is the least typical of all because ``aliens are not typically associated with cooking and pencils are not things that are typically cooked.'' 





\ex. \label{cook} \a.  \label{cooked1} The chef \textbf{cooked} the meal.
    \b. \label{cooked2} The waitress \textbf{cooked} the salad.
    \c. \label{cooked3} The alien \textbf{cooked} the pencil.


Then they rate three practice questions similar to \ref{cook} which they have to get right (rating the sentence like \ref{cooked1} above the midpoint, and those like \ref{cooked2}--\ref{cooked3} below the midpoint) to continue.   Then they rate eight calibration items, those found in our norming task to be closest to the Gaussian center, from among the normed ``handwritten control'' sentences (\S \ref{handwritten}).  Finally, they rate 89 more sentences which are a mix between a subset of the target items and a subset of the handwritten control items not used as calibration items, similar to the 89 used in the naturalness survey. A survey flow for both naturalness and typicality can be seen in Figure \ref{fig:surveyflow}.

\begin{figure}[h]
  \centering
  \input{figures/surveyflow}
  \caption{Survey flow for the naturalness, typicality, and pair difference tasks.}
  \label{fig:surveyflow}
\end{figure}


\begin{figure}[htbp]
  \centering
\includegraphics[width=1.0\textwidth]{figures/instr_exp2.png}
  \caption{Examples of how participants are prompted for their naturalness and typicality ratings, respectively. The modifiers of the endpoints of the scale differ because while the typicality of situations is not bounded, ungrammaticality of sentences is gradient judgement while grammaticality is not \citep{Pullum-Scholz-2001}.}
  \label{fig:instr_exp}
\end{figure}



Across all our studies, every sentence was rated by at least 5 annotators, all self-identified native English speakers located in the United States and recruited through the Prolific web platform.  No annotator was allowed to participate in more than one of these studies.  With IRB approval from our institutions, annotators were paid an average of \$12/hour.


%As an initial soundness check, Figure \ref{fig:nat} {\color{red} please see figure caption - would like 1 graph in total for naturalness, and 1 graph in total for typicality, each with 4 colors of dots} shows each sentence's mean rating (with each participant's responses $z$-scored by their own mean and standard deviation) as a function of its perplexity ({\color{red} TODO: cite perplexity OR maybe delete all this}), a measurement of how surprising each sentence is to a language model.  As predicted, sentences that are rated as more natural and typical have slightly lower perplexity.  This correlation is stronger for naturalness ratings than for typicality, which makes sense if we assume that the grammatical rules captured by naturalness are more inviolable than the stereotypical expectations captured by typicality.




% It follows that the more likely $w$ is given $c$, the less information it conveys, and it is thus read more quickly \cite{shannon}.   
 
% since it can calculate the likelihood of a token given its previous context. 
% Previous work has demonstrated that 
% We are able to use perplexity as a proxy for estimated human surprisal at a tokenized sequence because

% \begin{figure}[htbp]
%   \centering
% \includegraphics[width=\textwidth]{figures/heatmap.png}
%   \caption{Comparison of ChatGPT vs. PropBank's sense counts for the target verbs used in our studies.}
%   \label{fig:sense_comp}
% \end{figure}



\begin{table}[h]
\begin{tabular}{p{3.25cm} | p{6.5cm} | p{6.5cm} }
 & \textbf{Most natural}  & \textbf{Least natural}  \\ \hline
Corpus &  The people knew the truth. &The leviathan encountered the nothing. \\  \hline 
LLM + PropBank senses & The officer removed the suspect. &  The doctor set the nurse. \\ \hline 
LLM + LLM senses & \begin{tabular}[c]{@{}l@{}}The customer insulted the waiter.\\ The flood killed the crops.\\ The criminal murdered the victim.\\ The teacher removed the book. \\ The parent saved the child. \\ The judge understood the argument. \\ The child cleaned the toy. \\ The boy cleaned the room.\end{tabular}  & The package posted the mailbox. \\ \hline \hline
 & \textbf{Most typical}  & \textbf{Least typical}  \\ \hline
Corpus &  The staff cleaned the tables. &  The sign recalled the story. \\  \hline 
LLM + PropBank senses & The mechanic removed the tire. & The dog hacked the vet.  \\ \hline 
LLM + LLM's own senses & The plane reached the airport.  & The pet cleaned the carpet. \\ \hline \hline
 \end{tabular}

 \caption{Most and least natural and typical target sentences, according to our participants.}
\end{table}


\subsection{Analysis: Naturalness}
\begin{figure}[t]
  \centering
\includegraphics[width=\textwidth]{figures/point_naturalness.pdf}
  \caption{Mean naturalness rating for each sentences from each source. Each black point shows the mean rating of a sentence and large colored points show the mean of those means.}
  \label{fig:mean-nat}
\end{figure}
\subsubsection{Results}
Figure \ref{fig:mean-nat} shows the mean of z-scored naturalness ratings by generation process, and we intentionally separate the manually-generated calibration items by their naturalness and typicality. As expected, the manually-generated items that were both natural and typical are indeed rated as very natural. Furthermore, those manually generated to be unnatural were rated as such. Visually, the bar graph also shows that the target methods of comparison -- through using a corpus and our two LLM-based methods -- all generate items of similar naturalness. 


\subsubsection{Model fitting}

\begin{table}[]
    \centering
    \small
\begin{tabular}{rcccr}
\toprule
      & \textbf{Post. mean} & \textbf{2.5\%} & \textbf{97.5\%} & \textbf{Post.} $p$ \\
\midrule
Intercept & 2.24 & 1.63 & 2.84 & $<$ 0.01 \\
Manual (Typical \& Unnatural) & -2.75 & -3.36 & -1.95 & $<$ 0.01 \\
Manual (Atypical \& Natural) & -0.82 & -1.61 & -0.01 & 0.03 \\
Manual (Atypical \& Unnatural) & -2.91 & -4.12 & -2.02 & $<$ 0.01 \\
LLM with LLM-generated sense glosses & -0.52 & -1.15 & 0.06 & 0.04 \\
LLM with manually-generated sense glosses & -0.53 & -1.16 & 0.05 & 0.06 \\
Corpus & -0.31 & -0.99 & 0.31 & 0.22 \\
\bottomrule
\end{tabular}
    \caption{Fixed effect coefficient estimates for naturalness experiment with \textit{Manual (Typical \& Natural)} as the reference-level in a dummy coding. The 2.5\% and 97.5\% columns give the lower and upper bound of the 95\% credible interval, respectively, and the posterior $p$ column gives the posterior probability that the coefficient has the sign of the posterior mean.}
    \label{tab:my_label}
\end{table}

To confirm our visual conclusions, we use BRMS in R \citep{burkner} to fit a hierarchical Bayesian model (HBM) to examine the effects on ratings. HBMs are \textit{hierarchical} in that parameters can be organized into several layers and \textit{Bayesian} in that they make predictions about model parameters by updating prior beliefs with observed data to obtain posterior distributions.
While there are multiple ways to deal model distributions across a bounded, inclusive scale \citep{liukong2015}, we use a type of zero/one inflated beta (zoib) distribution since participants seemed to prefer the ends of the scale, leading to bimodality. 
Strictly speaking, a zoib is a mixture model that combines two models in order to handle the ends of the rating scale: a zero-one inflation component for the scale endpoints and a continuous beta distribution component for the non-endpoints of the scale. 
% -- specifically, an ordered beta \citep{kubinec_2020} -- 

We combine data from all three studies of naturalness in our first regression. The model predicts the log-odds of participants' rating of the naturalness of a sentence based on the following predictors: the generation procedure used to generate the sentence (LLM-generated with LLM senses, LLM-generated with Propbank senses, corpus-based, natural and typical manually-generated, natural and atypical manually generated, unnatural and typical manually generated, and unnatural and atypical manually generated), the centered log corpus frequency from COCA \citep{davies_2015}, the specific rater, as well as the verb, the sense of the verb, and the sentence, and their interactions.
We used uninformative default priors. The model converged, as indicated by all Rhats $=1.00$.
Full model summaries can be found in Tables \ref{tab:modelestimates-population-nat} and \ref{tab:modelestimates-group-nat} of the Appendix.

% The naturalness model's posteriors for different types of generation procedures can be seen in the left side of Figure \ref{fig:posteriors-nat}.
The model's intercept reflects the mean when all categorical predictors are at the reference level (i.e., the natural and typical manually-generated items) and the continuous predictors (i.e., the centered logged corpus frequency) are at 0, meaning that the frequency of the verb is at the mean of all frequencies.
With its $95\%$ Credible Interval (CrI) spanning $[0.75, 1.53]$, the model indicates that with $95\%$ certainty, the mean of ratings at this reference level in log-odds $1.14$ (out of log-odds space, this is $0.76$). This means that as we would expect, manually-generated items designed to be natural and typical are in fact rated as highly natural.

To consider the role of other generation procedure on ratings, we now focus on the posteriors for different types of generation procedures can be seen in the left side of Figure \ref{fig:posteriors-nat}.
Only for Natural \& Typical, Unnatural \& Typical, and Unnatural \& Atypical manually-generated items is the model 95\% certain that they have an association with ratings since these are the only levels that contain only positive or negative values in their CrI. 
Also expectedly, manually-generated items designed to be unnatural are in fact predicted to be rated as less natural than our reference level. 
Specifically, unnatural and typical manual items have a posterior of $-1.90$ log-odds ($95\%$ CrI: [$-2.30, -1.49$]) and unnatural and atypical manual items have a posterior of $-2.05$ log-odds ($95\%$ CrI: [$-2.58,-1.49$]). 
That the credible intervals are not near zero means that the model is quite confident on these parameters' effects on participant ratings.
In contrast, while the non-calibration items share visually similar posterior distributions, the model is not confident about these generation procedures' effect on naturalness ratings. 
Specifically, the model did not find a clearly positive or negative effect on ratings when compared to the reference level for LLM-generated items with LLM senses, LLM-generated items with Propbank senses, and corpus-generated items. 
% However, we can not conclude from this that the LLM-based and corpus-based procedures generated items of the same naturalness as our manual method, since the uncertain credible intervals are quite wide. 

Our naturalness model also considered the effect of centered log corpus frequency. The mean of this parameter's posterior is $-0.24$ log-odds ($95\%$ CrI: [$0.01,0.08$]). This narrow CrI suggests that the model is relatively certain that corpus frequency has a negative effect on participant ratings. However, the CrI bordering on zero means that the model considers very small and possibly null effects to also be plausible. In fact, it is this latter interpretation that better aligns with our predictions, since while we predicted that corpus frequency would be positively associated with typicality, we would not expect an association with naturalness either way.

Turning to the group-level predictors, our model estimates that the standard deviation for the intercept of the Rater ID parameter to be $0.41$ log-odds ($95\%$ CrI: [$0.36,0.47$]). This means that there is variability among raters in their baseline tendency to assign ratings, beyond what can be explained by the fixed effects in the model. Slightly wider, and thus more uncertain, is the posterior estimate for the standard deviation of the Verb parameter, which has a mean of $0.16$ and a $95\%$ CrI of [$0.09,0.23$]. This suggests that there is also by-verb variability in how they are rated by participants. However, the effect is quite small. Furthermore, the interaction between Verb and Sense (Verb * Sense) (posterior mean of sd(Intercept): $0.25$; 95\% CrI: [$0.19,0.31$]) as well as the three-way interaction in Verb * Sense * Sentence (posterior mean of sd(Intercept): $0.32$; $95\%$ CrI: [$0.27,0.37$]) also express a variability among ratings. This means that each generation procedure produces items with varying levels of naturalness.


% Since we want the outcome variable to fall between $0$ and $1$, inclusive, we divide \texttt{Rating}$/100$ and predict this value with  \texttt{Generation} (takes on values ``handwritten'', ``corpus,'' ``llm\_propbank'', ``llm\_nonpropbank'', respectively) as a fixed effect, \texttt{Rater\_ID} as a random intercept to consider by-rater effects, by-\texttt{Sense} random intercepts nested under \texttt{Verb}, and by-\texttt{Sentence} as a nested random intercept under \texttt{Sense} and \texttt{Verb}. We used uninformative default priors and consider an effect to be significant if $0$ is not included in the credible interval. Full model summaries can be found in Figure xx of the Appendix.

% The estimated intercept $\beta_0$ for our model transformed out of log-odds space is $0.515$ with $CrI=[-0.14, 0.26]$. Since the $95\%$ credible interval includes $0$, however, there is not enough evidence to conclude that the intercept is different from zero. 
% Ordered from the least increase to the greatest increase, participants are predicted to give significantly higher ratings when \texttt{Generation}==``corpus'' (hereafter in log-odds space, $\beta_1=0.94$ with $CrI=[0.72,1.17]$), then \texttt{Generation}==``chatgpt\_nonpropbank'' ($\beta_2=1.22$, $CrI=[1.00,1.44]$), then \texttt{Generation}== ``chatgpt\_propbank'' ($\beta_3=1.31$, $CrI=[1.09,1.54]$), compared to the baseline level at which \texttt{Generation}==``handwritten''. 
% These results demonstrate that at least when regarding the item generation process, participants generally found all three generation processes to produce equivalently natural sentences, which is expected given that they all had the same syntactic structure and thus any abnormality in naturalness arises from semantic processes such as selectional restrictions of the verbs. {\color{red} TODO: I still do not understand from this description, are the corpus/ChatGPT sentences MORE NATURAL than the handwritten sentences, or just EQUALLY NATURAL?}

% Regarding group-level effects, the estimated standard deviation (sd) of the intercept across $186$ levels of \texttt{Rater\_ID} is $u_{\text{rater\_id}}=0.43$, with $CrI = [0.37,0.49]$. This indicates that there is a fair amount of variation in the intercept across different raters, which provides our motivation for \textit{z}-scoring ratings by-participant in Figures xx. Furthermore, the sd of the intercept across $92$ levels of \texttt{Verb} is $u_{\text{verb}}=0.25$, with $CrI=[0.18,0.33]$. The sd of the interaction between \texttt{Verb} and \texttt{Sense} is estimated to be $u_{\text{verb:sense}}=0.18$ ($CrI=[0.07,0.27]$), indicating variation between the $375$ levels of interactions. Finally, the estimated sd of the interaction between \texttt{Verb}, \texttt{Sense}, and \texttt{Sentence} is $u_{\text{verb:sense:sentence}}=0.47$ ($CrI=[0.43,0.51]$), once again indicating variation across $1797$ levels. These effects demonstrate that the generated items' typicality is modulated by the specific sentences the most out of the nested mixed effects, since the last mentioned variation is around twice the magnitude of the others and has the highest CrI.  {\color{red} TODO rewrite/shorten this paragraph to use fewer numbers or at least put them in parentheticals; structure sentences around the plain English takeaway.}


\subsection{Analysis: Typicality}
\subsubsection{Results}
\begin{figure}[t]
  \centering
\includegraphics[width=\textwidth]{figures/point_typicality.pdf}
  \caption{Mean typicality rating for each sentences from each source. Each black point shows the mean rating of a sentence and large colored points show the mean of those means.}
  \label{fig:mean-typ}
\end{figure}
The mean typicality ratings by-Generation procedure can be seen in Figure \ref{fig:mean-typ}. Notably, the non-manually-generated items have lower means than in the naturalness task. Furthermore, items that were designed to be typical (but were also unnatural) were rated low for typicality. This suggests that the effects of unnaturalness can ``leak'' into perceptions of typicality. Now we turn to our model results to affirm and deepen our observations.

\subsubsection{Model fitting}
Just as we did for Naturalness, we fit a similar regression using data from all three Typicality studies predicting model ratings as a function of generation procedure, corpus frequency, surprisal, rater ID, verb, verb-sense, and sentence. Full model summaries can be found in Figures \ref{tab:modelestimates-population-typ} and \ref{tab:modelestimates-group-typ} of the Appendix.

Once again, the model's intercept reflects the reference level, which is the natural and typical manual generation method with zero centered logged corpus frequency. The model indicates that with $95\%$ certainty, the mean of ratings at the reference level is $1.18$ log-odds (out of log-odds space, this is $0.76$) with a $95\%$ CrI
 of $[0.88,1.48]$. Considering the other generation methods (visually depicted on the right side of Figure \ref{fig:posteriors-nat}), we can see that this typicality model predicts stronger effects of generation type, compared to our model for naturalness, since none of the distributions contain $0$. 
 Specifically, LLM-generated items with LLM senses (posterior mean: $-0.84$ log-odds; $95\%$ CrI: [$-1.15,-0.53$]), LLM-generated items with Propbank senses (posterior mean: $-0.72$ log-odds; $95\%$ CrI: [$-1.04,-0.40$]), and corpus-generated items (posterior mean: $-0.82$ log-odds; $95\%$ CrI: [$-1.14,-0.49$]) appear to have visually similar posterior distributions. Specifically, the model predicts each to have a negative effect on ratings when compared to the reference level of natural and typical manually-generated items.

 The model is even more certain about the effects that the natural and atypical, unnatural and typical, and unnatural and atypical manual generation has on participant ratings of typicality, since these posterior distributions are even further from zero that the non-manual generation procedures. 
 Specifically, natural and atypical manual items have a posterior mean of $-2.14$ log-odds ($95\%$ CrI: $[-2.53,-1.73]$) and unnatural and atypical manual items have a posterior mean of $-2.17$ log-odds ($95\%$ CrI: $[-2.87,-1.51]$). This means that these two generation procedures have a negative effect on typicality ratings, which aligns with what we expect since we purposely designed these items to be atypical. 
 Unexpectedly, however, those items we designed to be typical but unnatural were also predicted to have a negative effect on ratings (posterior mean: $-1.82$ log-odds; $95\%$ CrI: [$-2.39,-1.26$]). This aligns with what we observed from Figure \ref{fig:mean-typ}.

 Furthermore, the mean of the centered log corpus frequency is $0.09$ log-odds ($95\%$ CrI: [$0.04,0.13$]). That the $95\%$ CrI is comprised of only positive values suggests that there is a $95\%$ probability that this effect is positive, when all other predictors are at their means. Thus, we can be fairly certain that ratings of typicality are higher for verbs that appear more frequently in corpora, which aligns with our predictions.

 Turning to the group-level parameters, we find that similarly to the naturalness model results, there is variability among raters in their ratings of typicality. The model estimates the posterior mean of the standard deviation of Rater ID to be $0.28$ log-odds, with a $95\%$ CrI of [$0.24,0.32$]. The same variability from the naturalness models is also observed for the typicality model's estimates of Verb parameter (posterior mean of sd(Intercept): $0.20$ log-odds; $95\%$ CrI: $[0.12,0.28]$), as well as the interaction between Verb and Sense (posterior mean of sd(Intercept): $0.33$ log-odds; $95\%$ CrI: $[0.27,0.39]$), as well as the interaction between Verb, Sense, and Sentence (posterior mean of sd(Intercept): $0.55$ log-odds; $95\%$ CrI: $[0.51,0.59]$). 

 
% The estimated intercept $\beta_0$ for our model transformed out of log-odds space is $0.483$ with $CrI=[-0.09, 0.35]$ {\color{red} TODO please explain what the intercept means}.
% Ordered from the least increase to the greatest increase, participants are predicted to give significantly higher ratings when \texttt{SentenceSource}==``corpus'' (hereafter in log-odds space, $\beta_1=0.46$ with $CrI=[0.18,0.75]$), then \texttt{Generation}==``llm\_nonpropbank'' ($\beta_2=0.62$, $CrI=[0.34,0.91]$), then \texttt{Generation}== ``llm\_propbank'' ($\beta_3=0.74$, $CrI=[0.46,1.03]$), compared to the baseline level at which \texttt{Generation}==``handwritten''.  These results demonstrate that at least when regarding the item generation process, participants found all three target generation processes to produce items of similar typicality, more typical than the calibration items.

% In regards to group-level effects, the estimated standard deviation (sd) of the intercept across the $185$ levels of \texttt{Rater\_ID} is $u_{\text{rater\_id}}=0.28$, with $CrI = [0.23,0.32]$. This indicates that there is a fair amount of variation in the intercept across different raters. Furthermore, the sd of the intercept across $94$ levels of \texttt{Verb} is $u_{\text{verb}}=0.31$, with $CrI=[0.22,0.40]$. The sd of the interaction between \texttt{Verb} and \texttt{Sense} is estimated to be $u_{\text{verb:sense}}=0.34$ ($CrI=[0.26,0.41]$), indicating significant variation between the $377$ levels of interactions. Finally, the estimated sd of the interaction between \texttt{Verb}, \texttt{Sense}, and \texttt{Sentence} is $u_{\text{verb:sense:sentence}}=0.60$ ($CrI=[0.56,0.65]$), once again indicating significant variation across $1797$ levels. These effects demonstrate that the generated items' typicality is modulated by the specific items' verb and sense. {\color{red} TODO please insert plain English takeaway; also rewrite/shorten this paragraph to use fewer numbers or at least put them in parentheticals, focusing instead on the qualitative takeaways}

% {\color{red} TODO please insert plain English section summary}

